How Crucial Is It for 6G Networks to Be Autonomous?

The sixth generation (6G), unlike any of the previous generations, is envisioned by 2030 to connect everything. Moreover, in addition to the new use cases, 6G is expected to support, it will need to provide a superior performance over 5G. The global connectivity, large network dimensions, users heterogeneity, extremely low-power consumption, high throughput, ultrahigh reliability, efficient network operation and maintenance, and low-latency requirements to be met by future networks inevitably necessitate the autonomy of 6G. Intelligence, facilitated mainly by the advancement of artificial intelligence (AI) techniques, is a key to achieve autonomy. In this paper, we provide a bird's-eye view of 6G, its vision, progress, and objectives. Furthermore, we present some technologies that would be mainly enabling intelligent globally connected world. In addition to discussing the role of AI for future wireless communications, we, unlike any other review papers, provide our original results which give early evidence for the viability of achieving 6G networks autonomy through leveraging AI advances. Furthermore, we, very importantly, identify 6G implementation challenges and key innovative techniques that promise to solve them. This article serves as a starting point for learners to acquire more knowledge about 6G and also for researchers to promote more development to the field.

==> 6GVision.tex <==
% The  6G is depicted, in its first global vision,  as a framework   of different services such as sensing, computing, caching, imaging, highly accurate positioning and mobility, radar and navigation  integrated with the main communication services the previous generations provide. 
% 6G will be an autonomous-intelligent ecosystem connects everything through multi-dimensional  networks that provide services in the ground, air, space,  and underwater aiming  to provide quality of not just service but life. Benefiting from smart sensory environments, 6G will be driven by a variety of verticals including factories, automation and transportation,  and healthcare. 
% %This framework will be the key enabler to the vision of connecting everything to achieve a high-quality smart living with its ability to support full-vertical applications. \\
% 6G is predicted to be motivated by potential-new applications  
%  for which the currently deployed 5G infrastructure is not expected to support~\cite{saad2020avision}.
% A main domain of these applications is the connected robotics and autonomous systems that include self-driving cars, drone delivery systems, autonomous robotics.  These applications will get the full use of the multi-dimensional network structure and artificial intelligence  {(AI)} capabilities to be offered. Other  domains include extended reality  {(XR)}, blockchain and wireless brain-computer interaction based applications.  Different requirements for these use cases set different trends and research directions towards 6G. For example, some of these applications are bandwidth-intensive and thus require opening up new and wider spectrum such as terahertz  {(THz)} bands~\cite{chaccour2021seven}. Other applications require multiple small devices that mainly work on batteries and thus set the trend to develop highly energy efficient communications. More details about the  requirements demanded, and technologies promising for realizing the 6G are presented in this article. 

% . This will provide acceptable QoE for such scenarios as hyper-high-speed railway and airline systems 
% 6G will be an autonomous ecosystem with human-like intelligence and consciousness. It will evolve from human-centric to both human- and machine-centric, and it will provide multiple ways, such as through fingers, voice, eyes, and brainwaves (or neural signals), to communicate and interact with smart terminals." zhang2019
% Massive Internet of Things (IoT) and fully autonomous vehicles [6].support underwater and space communications industrial Internet 
% support the Internet of Nano-Things and Internet of Bodies 
% ~\cite{zhang20196G}
% %%%%%%
% "A number of new communication scenarios in future networks around 2030 are predicted in [4], which encompass holographic calls, flying networks, teleoperated driving, and the tactile Internet. [4] 
% [4] A.Yastrebova,R.Kirichek,Y.Koucheryavy,A.Borodin,andA.Kouch- eryavy, “Future networks 2030: Architecture & requirements,” in Proc. IEEE ICUMT, Moscow, Russia, Nov. 2018, pp. 1–8,
% "
% ~\cite{dang2020should}




















==> ChallengesAndSolutions.tex <==
\subsection{Complexity} 
 The superior performance of 6G and the ability to achieve full autonomous networks requires high computation capabilities, which will be a challenging task even for most powerful computers.  
Despite its extremely wide spectrum, mmWave and THz bands for example require highly directional transmission. This means searching in a very large angular space is essential for achieving high beamforming gain and thus, reducing the initial access  performance. In other words, the process of  aligning  two beams between two communicating entities out of  a set of many possible beams leads to so much overhead. 
From this, an ML and DL-based initial access method 
%using recurrent neural networks (RNNs) 
in mmWave communication was studied in~\cite{Mazin2018Accelerating,Myers2020Deep}. % :(
Moreover, the immense power of quantum computers in speeding up ML algorithms can be investigated not only for beam alignments, but also for users tracking,  learning and predicting locations~\cite{syed2019Quantum}. \\
 NOMA, even though it promises for high connectivity, it is still limited by the high computation complexity incurred for SIC  estimation  especially for a large number of users as stated earlier. Moreover, user clustering and power allocation in mmWave-NOMA demand high computational power,  as they need to be updated in real time. Emerging  AI techniques can overcome some of these limitations~\cite{Benfaid2021thesis,cui2018application}.\\ 
%  \blue{ UAVs on the other hand provided more mobility and freedom to the network and resource allocation, however, controlling such a network won't be an easy task, especially when considering a network of UAVs that provide service to ground users while switching packets between each other, they also should handover users to each other whenever a cell edge user is causing low overall system performance. An efficient solution has to be made in order to handle such multi-dimensional complexity, and since this problem is definitely non-convex, AI will be the number one candidate to solve such a complex problem}  \\
 %In the context of detection in NOMA, ML approach was proposed in [230]. In addition, ML for optimal user clustering and power allocation in mmWave NOMA was proposed in[231]
With the ever-increasing demand for high capacity, implementing multi-user multiple input multiple output (MU-MIMO) will be impractical. The utilized detection algorithms suffer from high complexity which increases exponentially with the number of users and data rate.~\cite{kim2019leveraging} is one of the few works
that proposed a solution for MU-MIMO complexity problems and showed its effectiveness by implementing it on a real quantum computer.
With very low bit error rate  considering different modulation schemes and channel conditions,  the authors of the paper managed to achieve MU-MIMO signal detection for number of users and data rates that are unfeasible to handle in  classical computers just  {in order of microseconds}.\\
%The authors of the paper managed to achieve signal detection in MU-MIMO for number of users and data rates that are unfeasible to handle in  classical computers, with very low bit error rate  in different modulation schemes and channel conditions {in just $10$µs}.\\
The necessity for high computational power and parallelism suggests that quantum machine learning (QML) can be a crucial candidate in 6G networks and beyond~\cite{syed2019Quantum}.\\

 %%%%%%%%%%%%%%%%%

\subsection{Security}
%Communications like industrial, health related application 
Number of applications including autonomous system such as healthcare, robotic, and vehicular communications demand a very-high level of security. Classical cryptographic methods would fail short with the emerging quantum technology~\cite{chen2016classCrypRept}. 
    Through some of its attributes including anonymization, decentralization, and untraceability, blockchain technology, however, can come as a solution for security vulnerability issues~\cite{henry2018blockchain}. 
    UAVs for example are emerging not just as aerial BSs, but also to provide a variety of other applications such as logistics, surveillance, disaster management, and rescue operations. Securing such UAV networks which will eventually be transformed into  Internet of UAVs, will inevitably require leveraging of  blockchain technology.
    Addressing   security issues  for which the unique 6G network may be vulnerable to, will certainly  require a lot of attention from the  research community. 


%  issues and solution: Machine learning for wireless connectivity and security of cellular-connected UAVs .. challita2019machine
%  [5] and [6] \cite{dang2020should}
 
 
 
% \subsection{Network Decentralization}

% blockchain.. 

% \red{will give Anas some more time ..until I wrap up the rest..otherwise will be included during the review process.. hopefully..  }


==> NOMA.tex <==
 {Traditional orthogonal multiple access (OMA) schemes
may struggle to accommodate the massive number of 6G connections, since  these techniques divide frequency resources to {weak and strong users}  equally.  
 {On} the contrary,  NOMA supports multiple users in the same time/code/frequency domain,
hence promises for better spectral efficiency and throughput.
%to meet the requirements of 6G networks.
Furthermore, OMA prefers users with good channel conditions which have higher schedule priority. However, in NOMA, users are served simultaneously.  Hence it offers    better fairness,  low{er} latency, and higher connectivity density.} To transmit two messages or more in the same time/code/frequency domains, NOMA uses superposition coding (SC) in the power domain~\cite{ding2017survey}, which aims to encode them into a single signal each of which get{s} assigned  {a} different power value depending on  intended receivers\textquotesingle~channel conditions. {Many users can be distinguished from one another at NOMA receivers by using successive interference cancellation (SIC).} %As a result,  {the} number of subscribers can be multiplied by a factor of ten or even more, making NOMA a promising scheme for future networks.}


NOMA, nonetheless, has some limitations, such as receiver computational complexity,  BS channel state information (CSI) prior knowledge, and performance {degradation} as \benfaid{the} number of users increases.
%,  which made the 3rd Generation Partnership Project (3GPP) defer it for beyond 5G networks after it has been considered as a study-item for 5G new radio (NR)~\cite{makki2020survey}.
Consequently, the 3rd Generation Partnership Project (3GPP) has deferred the use of NOMA for next\benfaid{-}generation networks, where most of these limitations will not be a concern, and given up \benfaid{\cancel{in} on} making NOMA an option for 5G~\cite{3GPP2018noma5GNR,makki2020survey}.   
%\red{note about the original reference 3GPP needs to be cited and can in addition we can cite makki2020survey in case we believe there more evidence in that regard etc..}
%\blue{notice I did the same for the pencil beams.. I skimmed over the reference you have included tan2020thz and realized that  rappaport2019wireless was the original .. I cited both the original and  tan2020thz which invistgated more on the idea of   rappaport2019wireless}  

 { To benefit from the superiority of NOMA  in fairness, latency, throughput, and connection density in the 6G networks\benfaid{,} however, it will \benfaid{be} expected to be merged      with mmWave to get the best of both worlds in 3D networks, which  utilizes aerial base stations.
 %\red{will need to double check what we discussed regarding 3d networks in above 6g tech. subsection as it should of stated why 3D}
 Handling such a network, nonetheless, would be a complex non-convex problem \benfaid{\cancel{which} that} traditional mathematical solutions can not solve, however, we will discuss how to viability of  managing these networks autonomously  by using the power of AI.} 
 
 
%\blue{we may  indicate somehow how why beyond 5G can solve the issue by relating the 3D network to 6G ..} \red{if not clear, I will take care of it as it is not crucial for you to do it}
 
 %and their channel gains become comparable. %
%from the superiority of NOMA over OMA techniques,
%in fairness, latency, throughput, connection density as well as compatibility,
%number of solutions are proposed in the literature to some of the aforementioned challenges 
%There has been some efforts to use NOMA for 5G new radio (NR) which has been considered as a study-item in 3GPP, however, it has been deferred for beyond 5G~\cite{makki2020survey}.
%A way, an essential one, to improve is to structure the subsection or think of the current structure and see what changes should need to be made .. how are thoughts or ideas flow or should flow..

% \noindent{NOMA's advantages over OMA can be summarized as follows:}
% \begin{itemize}
%     \item Spectral efficiency and throughput.
%     \item User fairness, low latency, and massive connectivity.
%     \item Compatibility.
% \end{itemize}

%In OMA, frequency resources are divided equally to the strong and weak users, however, in NOMA, the weak and strong users share the same frequency resources hence better resource efficiency. Which will yields better spectral efficiency and throughput. Furthermore, OMA prefers users with good channel conditions which have higher schedule priority compared to OMA, however in NOMA, there are no such waiting time, hence better fairness and low latency, and massive connectivity. Since NOMA does not necessitate significant changes to the existing architecture, NOMA is therefore compliant with present and future networks. In other words, OMA's insufficient performance leaves it inapplicable and unsuitable for delivering the features needed by 6G. Despite NOMA advantages, it still has some limitations, such as receiver computational complexity, channel state information (CSI) is required to fed back to the BS, the error probability of the SIC is increased whenever more users are connected which will limit the number of users, and channel gain differences among all users is required to have a better network performance.
%"The need for privileging the access of wireless medium to a massive amount of users in an ultra-efficient fashion has led to the evolution of multiple- access mechanisms. Conventionally, the orthogonalization has been achieved through a clear distinct allocation of resources to the users through slicing of available resources in time, frequency, code, or space domains. With an increase in users, the mechanism for spatial re-utilization of the resources emerged, which further evolved into the idea of cognitive radio. As of today, a further massive increase in the number of network users/devices is causing the transition from conventional orthogonal multiple access methods to (random) NOMA methods. The NOMA scheme utilizes an additional domain of power, while it mostly revolves around the hybrid of different conventional orthogonal multiple schemes, i.e., division in joint multi-dimensional space of power, angle, and code etc. In NOMA, advanced signal processing methods are exploited to suppress the interference in order to accurately decode the data symbols, e.g., SIC. The hardware support for such SIC at user nodes is also released as NOMA-chipset [226]." Syed2019

==> Progress.tex <==


%Recently, as the the 5G standard has been getting finalized,  researchers from industry and academia have begun to envision the 6G communication networks 


==> Quant.tex <==


 
Quantum-assisted communication is a novel field that can be viewed  as one of the cornerstones for future multi-state networks. Rendering to their capabilities in solving problems exponentially faster than their classical counterparts,  
quantum computers (QC) will \benfaid{\cancel{be}} bring \benfaid{a} new era in  telecommunication. Their working principle is based on essential concepts of quantum mechanics such as superposition, entanglement, and no-cloning theorem~\cite{Gyongyosi2019Survey}.% \red{just to make this reference should explain all the aforementioned concepts (superposition, entanglement, and no-cloning)}
Constructing independent copies of quantum information  is impossible, as the no-cloning theorem states. Thus, offering high communication security which should be a key feature of 6G.
%quantum information (qubit)
A qubit,  quantum analogy of  classical bit,  represents a two-level quantum system, where each level is called a state. Instead of representing zero or one only, however,  a qubit can be in a linear combination (or superposition) of both. That means upon measurement, a qubit will be found with some probability in the one or the zero sate. 
For n qubits, a quantum computer can work with $2^n$ quantum states simultaneously.  This parallelism makes quantum computers potentially useful in applications that require the processing of big data. Many efforts have been done by the research community to investigate on the involvement of quantum speedups in various communication areas. The authors in~\cite{botsinis2019Quantum} for instance  {have proposed and presented}  a number of quantum search algorithms that are particularly applicable to wireless communications. Quantum computing merged with different AI techniques (e.g., quantum machine learning) has promising potentials in solving challenges in many aspects of 6G networks and beyond~\cite{syed2019Quantum}.   


%the potentials of QC and discussed different research directions in merging quantum computing with several AI techniques in 6G networks as well as open research problems in the field.  \red{still not general enough as it focuses on the reference ..}
%\red{sounds great ..one more thing though, can you end the subsection more generally? a possible way could be separating the two last   clauses the one related to ref:botsinis2019Quantum  could be used as an example for the efforts done in wireless communication.. the other reference could be used in more general way to end the subsection for example indicating the future of  quantum and its promises when combined with AI in solving and the fact there still way more to do in the field (quantum communications) as it is in its infancy we may say why.. }
%For instance, quantum search algorithms in wireless communications have been proposed in \cite{botsinis2019algor}. Also, authors in \cite{syed2019}   

 

==> UAV.tex <==
Aerial BSs, or UAVs,  are emerging as one  {of} the 6G essentials as they can provide high data rates and global wireless connectivity.  UAVs enjoy  exclusive features  such as ease of deployment, high LoS links probability, and large degree-of-freedom provided through their controlled mobility~\cite{li2018uav}.
 UAVs can be  deployed to offer wireless connectivity in case of  emergencies such as natural disasters,  overcome  last mile issues,   enhance capacity, replace terrestrial BSs, etc. 
 Allowing UAVs to  adaptively  relocate according to environmental changes and user demands, the 3D mobility is one of the most important UAV features.  
 %As an example, there might be dense users in certain locations that are far from the BS and relatively low density near it, in this case, terrestrial BSs can't do anything to make the system performance better, however, in UAV case, it can move towards the dense area in order to maximize overall system performance.
The goal of  connecting the unconnected to be met by the 6G will be made possible by the aerial BSs  as their deployment are much easier and more economical  than that of their terrestrial counterparts, especially in rural areas. 
%please double check if there is any redundancy with some thing that has been said previously
% the following looks fine
Rending to their ability  to connect with low earth orbit (LEO) satellites, CubeSats, and terrestrial BSs, UAVs  are also envisioned to  be one of \benfaid{the} main technologies to realize the 6G multi-dimensional network.  Managing UAVs\benfaid{\textquotesingle} placement and resource allocation simultaneously, however,  is a challenge that has to be addressed effectively in order to get the most out of their resultant 3D networks.   
AI advances  are promising, nonetheless, in managing the UAV networks effectively~\cite{Benfaid2021thesis}. % along with other innovative technologies like quantum computing
%\red{cite  thesis and AdaptSky as it gets announced ..}.
% In order to use the most out of UAVs to meet 6G requirements, further technologies like the mmWave .



==> UAVresults.tex <==
   Managing a networks that integrates mmWave, NOMA, and UAV technologies such that  the  power and beam  allocation, and UAV placement are jointly optimized, for example,  is definitely a complicated task and  traditional methods fall short to handle~\cite{Benfaid2021thesis}.  % non-convex 
 Using novel-AI solutions, we, nonetheless,  accomplished  in~\cite{Benfaid2021thesis} to not only solve the problem without the need {of} disjointing it into sub (unrealistic) ones but also  outperform some other existing heuristics derived  by legacy methods e.g.~\cite{Chen2019}. We, more specifically, proposed a  deep reinforcement learning (DRL)~\cite{mnih2013playing} based framework  that simultaneously places a  UAV in a 3D space  and allocates NOMA  power among users associated in clusters such that average sum of users\textquotesingle~data rate is maximized and certain fairness criteria is met. 
In this article, we present some of the simulation results as the UAV is being trained to learn the optimal decision while serving a total of four users, where each two are  associated with a certain cluster. The $ith$ user will be denoted by USERi and a decision interval will be referred to as an episode. 
More details about the framework and simulation setup are available in~\cite{Benfaid2021thesis}.
%A reader may refer to~\cite{Benfaid2021thesis} or \red{cite AdaptSky} for more details about the framework and simulation setup. 
Fig. \ref{fig: AdaptSky Clusters} shows power allocation, channel conditions, and average sum rate of our proposed framework, denoted by DRL, as they vary over episodes.  In Fig. \ref{fig: AdaptSky Clusters}(c) we include the average sum rate achieved by the state of art (SoA) suggested in~\cite{Chen2019} and denoted in the figure by SoA. 
%
 We can notice that the DRL average achievable sum rate converges to $23.5$ Gbit/s which represents a $57\%$ improvement compared to $15$ Gbit/s given by SoA. 
  To be able to determine a  mathematical solution for the optimization problem,  the authors in~\cite{Chen2019}  ended up restricting  the UAV  placement into  a 2D plane. In contrary, our DRL framework allows  3D UAV mobility without making any confines. Hence, the gain in performance our AI based technique offers is intuitive. 
  Furthermore, we can notice that DRL managed to recognize the NOMA power allocation users order by allocating the far user (the one with the poor channel condition as depicted in the top of  Fig. \ref{fig: AdaptSky Clusters}(a) and (b)) more power (as exhibited in the bottom of Fig. \ref{fig: AdaptSky Clusters}(a) and (b)) than the near one without even imposing that in the algorithm. The resultant choice of order is crucial for the work of SIC~\cite{ding2017survey} and is the best  to get the most out of NOMA. The  power allocation related decision was made intelligently and autonomously by the UAV through the careful algorithm design with the goal of  improving  total sum rate and maintaining a certain fairness level. 
The presented findings 
%and the decision process made through the proposed  framework,
do not only show how compelling  AI schemes are in enhancing performance, but also their abilities in  achieving autonomy and hence realizing  future network vision.

\begin{figure*}
     \centering
     \begin{subfigure}{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{AdaptSky-LoS-CLuster_1.pdf}
         \caption{}
         \label{fig: LoS-Cluster_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{AdaptSky-LoS-CLuster_2.pdf}
         \caption{}
         \label{fig: LoS-Cluster_2}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{AdaptSky-LoS-Clusters-Sum-rate.pdf}
         \caption{}
         \label{fig: LoS-Clusters-Sum-Rate}
     \end{subfigure}
        \caption{DRL decision and performance without forcing NOMA order (a) \& (b) cluster 1 \& 2 channel conditions and power allocation respectively, and (c) total average achievable sum rate~\cite{Benfaid2021thesis}.}
        \label{fig: AdaptSky Clusters}
\end{figure*}


% We present some  results from~\cite{Benfaid2021thesis} to which emphasize the benefits of using AI  in designing networks  that merge the mmWave, NOMA, and UAV technologies.
% The simulation has been done in a mmWave-NOMA environment  with a total of four users, where each two are  associated with a certain cluster as discussed in detail in~\cite{Benfaid2021thesis}.
%  One of the 6G trends would be to offering multi-dimensional networks where users (e.g. drones used for logistics) as well as BSs (i.e. UAVs) may  be located in the 3D space resulting in a 3D network.  Nonetheless,  managing  a 3D networks, optimally placing UAVs, and jointly allocating NOMA resources among users is definitely a complex non-convex task. 
%  It is impossible to solve such a problem using traditional mathematical solutions without oversimplifications.  However, using novel-AI solutions, specifically deep reinforcement learning (DRL)~\cite{mnih2013playing}, we managed to not only solve the problem without the need {of} disjointing the problem into sub (unrealistic) ones but also  outperform some other existing heuristics derived  by legacy method, for example the state of art (SoA)  provided by~\cite{Chen2019} which will be denoted as  SoA. 
% %
% %The core part of the proposed framework (which will be named AdaptSky throughout the paper) is Q-learning with neural networks as a model prediction, which is a framework that consists of four parts: agent, actions, states, and rewards. The main objective of this framework is to make the agent (in our case it is the UAV) learn a policy (set of actions given states) in order to get the maximum possible cumulative rewards (sum rate in our case). At each time step AdaptSky will do the following:
% %\begin{enumerate}
% %    \item Receive states from environment such as the users location, channel conditions, power allocation, and the UAV height.
% %    \item Take an action from the action state space corresponding to the states it received from the aforementioned step. The action state space consists of changing the users power allocation and the UAV placement.
%   %  \item As a result of the action a reward is received and the previous state is switched to a new one.
% %\end{enumerate}
% %

 
% Fig. \ref{fig: AdaptSky Clusters} shows power allocation, channel conditions, and average sum rate of a DRL training session against SoA.
% %
%  The baseline or SoA assumes the UAV can only be placed in  a two-dimensional plane in order to simplify the task, in contrary to our DRL framework which allows  3D UAV mobility without making any restrictions. We can notice that DRL average achievable sum rate converges to $23.5$ Gbit/s which represents a $57\%$ improvement compared to $15$ Gbit/s given by SoA. Furthermore, we can notice that DRL managed to recognize the NOMA power allocation users order by allocating the far user (the one with the poor channel condition as depicted in the top of  Fig. \ref{fig: AdaptSky Clusters} (a)) more power (exhibited in the bottom of Fig. \ref{fig: AdaptSky Clusters} (a)) than the near one without even imposing it in the algorithm. The  rule  of allocation order chosen  intelligently by the UAV, through the careful algorithm design, 
%  is important to   achieve fair allocation while improving the total sum rate over conventional access techniques.  \\
% The aforementioned results and the decision process made through the proposed  framework, do not only show how powerful the AI is, but also how necessary it is to be used in the next generation in order to achieve the 6G vision.


% %channel conditions as good as possible while giving the other user in that cluster approximately $70\%$ of the power to ensure that it gets the minimum spectral efficiency required $\bar{r}_{min} = 2.5$ bit/s/Hz to get the maximum achievable sum rate from all the users which is AdaptSky target at this scenario. We can see that the moving average for the total achievable sum rate for the last 100 episodes was approximately $\bar{R}_{t,1000} = 23.5$ Gbps  which represents a $57\%$ improvement compared to $\bar{R}_{t,100} = 15$ Gbps given by the first 100 episode moving average. 
 

==> blockchain.tex <==
Blockchain  is considered as a technology breakthrough in the recent years that is expected to have an important role in achieving 6G objectives~\cite{hewa2020therole,nguyen2020blockchain}. Blockchain is simply a database structure, %by definition,
it offers multiple key characteristics that are useful when used with certain applications. Blockchain stores data in blocks called datablocks, each datablock is attached to the previous one forming a chain of blocks. This chain is replicated and stored across different nodes that form a network. Once a data update request is initiated, it is broadcasted to all nodes where they use their available computational power to verify that it follows some pre-defined rules, once verified, the datablock is linked to the previous one in the chain. 
%
The described structure along with the operation method enable the blockchain technology to be used in applications that require high level of security, where changing one datablock in a certain node can be easily detected once the other nodes cross-reference each other. 
Other characteristics provided by blockchain-based systems are their scalability, where they can be used for 6G to overcome scaling limitations of centralized conventional networks. Transparency is also a key feature of blockchain that can be used for dynamic resource  management across different small scale operators since the records can be set to be accessed with equal rights without the need for a third party. The distributed  architecture of blockchain is also beneficial in facilitating decentralized systems and thus eliminating single point failures of previous generations systems.  

Consequently, blockchain was proposed to be used in different areas of 6G such as blockchain-based resource management frameworks~\cite{hao2020}, and blockchain-enabled architectures for UAV networks to ensure security and privacy with enhanced network performance~\cite{gupta2021}.
 

%The authors in \cite{hao2020} reviewed and compared multiple blockchain-based resource management frameworks, whereas the authors in \cite{gupta2021} proposed blockchain-enabled architectures for UAV networks to ensure security and privacy with enhanced network performance over conventional methods. 
 

 

==> spectrumtech.tex <==
The sub-6 GHz band becomes highly congested due to heavily used frequency resources. It  no longer can  support massive increases in communication capacity. 
Allowing accessibility to higher frequencies and bandwidth, the millimeter wave (mmWave) technology has been emerging to overcome the lack of spectrum issue\benfaid{s}.   Facilitating the 6G high-rate high-mobility use cases  (e.g. autonomous vehicles), mmWave is considered to be one of the 6G enabling technologies~\cite{chaccour2021seven}.  Owing to its ability to offer even more abundance of bandwidth, THz is also viewed as one of the very key 6G promising technologies.  
 MmWave communications, ranging from around $30$ GHz to $300$ GHz, {will} be one of the leading candidate systems for cellular mobile communications for future networks~\cite{xiao2017millimeter}. 
MmWave  can achieve peak data rates of $10$ Gbit/s or more with full-duplex capability, far exceeding the lower microwave frequency limit of $1$ Gbit/s~\cite{rappaport2017overview}.  
Despite its benefits, nevertheless, atmospheric absorption   highly  attenuate\benfaid{s} mmWave signals. 

  In order to measure the obtained power at the receiver $P_R$  with a distance $d$ apart from the transmitter and a signal wavelength  $\lambda$, we usually use the Friis Law~\cite{rappaport1996wireless}, which shows the relation between the received and the transmitted power $P_T$ for free-space propagation,  
  as shown,

\begin{equation}
\label{eqn: FSL}
    \frac{P_R}{P_T} = G_T G_R (\frac{\lambda}{4 \pi d})^2 
\end{equation}

Where $G_R~\&~G_T$ are the receiving and transmitting antenna gain respectively.  {The aforementioned equation works only in free space propagation, however, more generalized environments  
are discussed in~\cite{heath2016overview}.}
%and $n$ denotes the path loss exponent ($n = 2$ in the free space case).
We can notice from the equation 
%(\ref{eqn: FSL}) 
that under the same distance and antenna settings as microwave signals below 6 GHz, the free space path loss for mmWave signals is much higher. %, i.e. free space path loss increases as the signal frequency increases.
 This shows that using mmWave frequencies reduces the transmission distance which is a huge disadvantage in mmWave systems.
Due to their associated signals\benfaid{\textquotesingle} short wavelengths, nevertheless,  mmWave technology can be integrated with  large-scale multi-element antenna arrays allowing for high antenna gain and highly\benfaid{\cancel{-}}directional communications.  
% Furthermore, thanks to strongly directional signals and higher resolutions, short beams of mmWave signals increase security and interference immunity. 
 Innovative technologies  like super massive (SM) multiple input multiple output {(MIMO)}~\cite{yang20196g} along with the  beamforming techniques  are considered  to extend the transmission distance  and hence overcoming the shortcoming of using high frequencies.
 Thanks to the strongly directional communications  resulting from merging the aforementioned technologies, mmWave enjoys more security and interference immunity than that for lower \benfaid{\cancel{frequencies}} \benfaid{frequency} waves. \\
%
Another  major technical challenge, however, for mmWave is the blockage effect. 
%as mmWave signals get blocked by physical obstacles in their propagation paths. 
Rending to their abilities in providing  line-of-sight (LoS) links with a high chance,  aerial base stations (BSs) can decrease the impact of the aforementioned issue. 

Despite any of the concerns regarding the poor transmission properties of these wavelengths, commercial mmWave communications have become a reality with the standardization of 5G.
\\
Even if 5G solutions are still being deployed, there has been an argument that 5G's possible potentials would fall short of many new technologies, such as 3D gaming and XR.
%their gigabits per second speeds  its   
Hundreds of gigabits per second to multiple terabits per second data rates are needed for these applications which will require some other innovative solutions. \benfaid{\cancel{Which}} \benfaid{This} leads us to THz communications systems\benfaid{\cancel{,}} since they are widely recognized as the next step of wireless communications research due to their ability to deliver such data rates over short distances~\cite{chaccour2021seven}.
%
THz waves cover the frequency range of 0.1 to 10 terahertz. The 275GHz–3THz band spectrum is the main part of the THz band for cellular communications, according to International Telecommunication Union Radio Communication Sector (ITU-R) guidelines~\cite{stoica20196g}. \\
{Despite their features, there are many open research issues in THz radio systems such as small propagation range due to high propagation and molecular absorption losses, and THz transceiver design that will need to be addressed to make it realizable. However, to achieve a successful THz deployment and operation in 6G networks,
%next-generation wireless systems,
%some recommendations concluded by~\cite{chaccour2021seven}, such
pencil beams~\cite{tan2020thz,rappaport2019wireless} and holographic surfaces~\cite{huang2020holographic} are two of the main candidates to overcome THz issues.  
Nevertheless, the co-existence of THz systems with sub-6 GHz and mmWaves is necessary, especially in non-line-of-sight and mobility users cases, where the path loss would increase exponentially, which also gives the need of fusing machine learning (ML) techniques to make data-driven decision to get the best out of resources.}
In addition to the mmWave and THz technologies like optical and visible light communication (VLC)~\cite{saad2020avision} are some other above 6G non-radio frequency (RF)  spectrum technologies promising for capacity boosting.

%co-existence with sub-6 GHz and mmWave, and machine learning (ML) techniques. \red{please end more generally .. one suggestion could be to keep pencil beams \& holographic surfaces and provide original references for them.. we do not need to focus on references ..and add another sentence that is more general discussion about  the importance of merging technologies (sub-6G, mMwave, THz in ) in boosting  whiling adapting to face challenges including mobility e.g. and the importance of fusing ML to make data driven decision and get the best out of resources.. }
%what if indicate briefly that the loos solution  is to go with pencil beams this way we can end the subsection more positively (as we have tried to do previously with other subections..right? you may refer to Chaccour2021 )

%
%However, we can decrease the effectiveness of the aforementioned issues by using 3D aerial BSs (to be discussed later), which provide better line-of-sight (LoS) probability~\cite{lyu2016placement}. Furthermore, they can relocate to reduce interference.
%
%Despite any of \red{the concerns regarding the poor transmission properties} of these wavelengths, commercial mmWave communications have become a reality with the standardization of 5G.  \red{Even if 5G solutions are still being deployed}, many new technologies, such as 3D gaming and XR, are being argued that their gigabits per second speeds would fall short \red{of..}. Hundreds of gigabits per second to multiple terabits per second data rates with low latency and high efficiency  that are needed for these applications will require some other innovative solutions.

%The THz  has a frequency range that is too high for nowadays oscillators and too low for optical photon emitters, so it will be a challenge to design  transceivers in this range of frequency.


%The signal to be produced has a frequency range that is too high for nowadays oscillators and too low for optical photon emitters. The THz gap is the name for this problem and many other open research problems that still haven't been addressed yet which is out of the context of this paper. THz still a promising as mmWave has been one of the 5G enabling technology. 

 %Orbital angular momentum is another related capacity increasing emerging technology ~\cite{lei2015OAM,zhang20196G}.

%However, despite THz features, there are many open research issues in THz radio systems, such as smaller propagation range due to high propagation and molecular absorption losses. THz transceiver design where wideband is needed, is also a  significant challenge.  The THz gap is the name for this problem and many other open research problems that still to be addressed \red{cite..}.\\






 
% Current terrestrial network capabilities (technologies) are (very) far from /enough/ to satisfy 6G requirements for extremely broad coverage and ubiquitous connectivity. Therefore, a large-dimensional network integrating nonterrestrial and terrestrial networks is needed to support various applications, such as flight in the sky, voyage at sea, or vehicles on land.

% This works in the low-frequency, microwave, and mm-wave bands to provide more flexible and reliable connectivity for urgent events or in remote mountain areas by densely employing flying base stations (BSs), such as unmanned aerial vehicles (UAVs) [7], and floating BSs, such as high- altitude platforms. The location features of floating BSs can help connect space networks and reachable UAV BSs via the 6G-defined optical interface.

% "Network Capacity: Traditionally, the cell- densification strategy has been the prime enabler of increasing network capacity. However, shrinking the cell-size (e.g., tiny-cells) also requires suitable management of the increased inter-cell interference to the cell-edge users. With the rise of smart cities, mMTC, and mobile users on land as well as airborne, cell-densification through static BSs alone cannot meet the exponential growth in capacity demands. This problem can be alleviated by hybrid cellular networks employing Unmanned Aerial Vehicles (UAVs) as mobile BSs [59]. These UAV BSs can not only offload the data-traffic of the static BSs but they can also relocate dynamically to provide a more favorable propagation channel to the edge users. Also, the increasing demands on the frequency resources can be addressed by sharing the mmWave band between satellite and terrestrial communication networks to give a more global mobile coverage [60]. This 3-Dimensional (3-D) nature of the 6G coverage specifications has led to volumetric descriptions of spectral efficiency requirements in bps/Hz/m3. The introduction of mobile BSs and dynamic spectrum sharing have opened up the possibility of employing ML tools to optimize these new network parameters such as route optimization for the UAV BSs [59] or efficient spectrum sharing [61]." 
